SparsePose: Sparse-View Camera Pose Regression and Refinement

Camera pose estimation is a key step in standard 3D reconstruction pipelines that operate on a dense set of images of a single object or scene. However, methods for pose estimation often fail when only a few images are available because they rely on the ability to robustly identify and match visual features between image pairs. While these methods can work robustly with dense camera views, capturing a large set of images can be time-consuming or impractical. We propose SparsePose for recovering accurate camera poses given a sparse set of wide-baseline images (fewer than 10). The method learns to regress initial camera poses and then iteratively refine them after training on a large-scale dataset of objects (Co3D: Common Objects in 3D). SparsePose significantly outperforms conventional and learning-based baselines in recovering accurate camera rotations and translations. We also demonstrate our pipeline for high-fidelity 3D reconstruction using only 5-9 images of an object.

==> fig/camupdates.tex <==
\begin{figure}
\centering
\includegraphics[width=0.9\columnwidth]{fig/\currfilebase}
\caption{\textbf{Camera updates} -- \TODO{figure that shows camera getting updated from initial poses to final poses}}
\label{fig:\currfilebase}
\end{figure}

==> sections/03_background.tex <==


\section{Background}
\label{sec:background}
% \subsection{Notation}

\AT{consider making this a subsection of related works? or a subsection of method. And after reading, this goes in method, as you are framing the problem.}
\Sam{I usually like a separate background section... but dont have any strong attachment to it}

\DL{This section seems out of place to me... I think it would be better to proceed with the methods section directly. For example, the first paragraph here could easily go into the methods, and the second paragraph might not be necessary at all.}

\paragraph{Camera Pose Estimation}
% 
Given a set of $N$ source images~$\{\image_n\}{=}\{\image_1, \dots, \image_N\}$, the goal of camera pose 
% \AT{pose usually == extrinsics, here it's just camera no?} 
% \Sam{we only predict extrinsics and rely on gt / colmap intrinsics - which is usuaully pretty reasonable since phone have their gt intrinsics} 
estimation is to predict the intrinsics camera parameters (focal length, principal point and skew) and extrinsic location and orientation.
% \AT{can we drop ``src''? we can just assume $\image$ stands for source image, no? This lightens notation}
In this paper, we only consider the task of estimating \textit{extrinsics}; we assume the intrinsics are known as they can be calibrated once for a camera a priori or are often provided by the camera manufacturer. 
% More formally, the goal of this paper to predict $n$ rotations $\mathbf{R} \in \mathrm{SO}(3)$ and translations  $\mathbf{T} \in \mathbb{R}^3$ given $n$ source images $\{\mathcal{I}_{src}^n\}$.
More formally, our goal is to jointly predict the set of rotations~$\{\rot_n {\in} \mathrm{SO}(3)\}$ and translations~$\{\tra_n {\in} \mathbb{R}^3\}$ corresponding to the source images~$\{\image_n\}$.

% \todo{Camera pose estimation is a necessary step for most 3D reconstruction pipelines, since most algorithms learn the 3D structure of the scene using the estimated camera poses.}
% \AT{drop, this reads like it belongs in intro}

% Typically, Structure-from-Motion (SfM) is a popular technique to recover the 3D geometry of a given scene.
% Such methods, such as COLMAP \cite{sfm_revisited}, refine the camera pose estimates using epipolar geometry and a non-linear
% optimization technique known as ``bundle adjustment''.
% Bundle adjustment works by minimizing the re-projection error:

% Structure-from-Motion (SfM), e.g. COLMAP~\cite{sfm_revisited}, is a popular technique to recover the extrinsics of a scene by refining camera pose estimates via ``bundle adjustment'' \AT{bundle adjustment also co-optimize the latent 3D points, not just the pose, no? I think your equation is incomplete?}:
% % 
% \begin{equation}
%     \min_{P} \sum_{i,j} v_{i,j} \cdot d(P_j X_{i}, x_{i,j})
% \end{equation}
% % 
% a non-linear optimization that minimizes the re-projection error of points with similar appearance.
% % 
% % Typically, Structure-from-Motion (SfM) is a popular technique to recover the 3D geometry of a given scene.
% % Such methods, such as COLMAP \cite{sfm_revisited}, refine the camera pose estimates using epipolar geometry and a non-linear
% % optimization technique known as ``bundle adjustment''.
% % Bundle adjustment works by minimizing the re-projection error:
% % 
% % 
% % \begin{equation}
% %     \min_{P} \sum_{i,j} v_{i,j} d(P_j X_{i}, x_{i,j})
% % \end{equation}
% % 
% \todo{where $P_j$ is the $4 \times 4$ world-to-camera projection matrix in homogenous coordinates for the $j$-th source image in 
% $\{\mathcal{I}_{src}^n\}$, $X_i$ is the $i$-th 3D point, $x_{i,j}$ is the actual projection of $X_i$
% onto the $j$-th source image and $v_{i,j}$ is a simple binary scalar that denotes whether point $X_i$ is visible in the 
% $j$-th source image.
% $d(.,.)$ is a distance function such as Euclidean distance or a more robust distance function variant \cite{robust_l2}.
% Simply, bundle adjustment aims to refine the camera pose estimates by projecting 3D points onto each of the source images
% where the point is visible, and minimizing the error in the predicted projection given by $P_j$.}
% \AT{are you re-using all of this math later on? if not, skip it}
% \AT{if you want to keep it, this is the place where you formalize how rotation and translations are put together into a homogeneous transformation $\mathbf{T}$}

\paragraph{Neural Radiance Fields}
% 
Neural Radiance Field~\cite{nerf}, or NeRF, have become increasingly popular in representing the 3D geometry and texture of the scene.
Such methods use coordinate neural networks to encode the scene and are trained to predict the colour $c \in \mathbb{R}^3$ and opacity $\sigma \in [0,1]$ given a 3D point $\mathbf{X} \in \mathbb{R}^3$ and the camera viewing direction $\mathbf{d} \in \mathbb{S}^2$.
The scene is parameterized using Multi-Layer Perceptrons (MLPs), and is typically \textit{overfit} to a single scene.
In practice, NeRFs use \textit{positional encodings} to encode the 3D coordinates before they are passed to the MLP, which can be expressed as $\gamma(a) = [\sin(x), \cos(x),\dots,\sin(2^N x), \cos(2^N x)]$, where $N$ is a hyperparameter, and $a$ is any raw 3D coordinates.
\AT{too much detail, yet too little motivation -- if you really want to highlight posenc, then you need to say why they are used... to overcome the spectral bias of MLPs and let them overfit well to a signal. But do you really need to write equations? Not unless your model tweaks them in some way.}
\Sam{the reason i mention positional encoding for example, is because i use it in the methods section, and its rather easy to explain here.
BTW: this is the $\gamma(.)$ you asked about in eqn 4.}
\AT{too far, just mention it where it's used -- ``and we use gamma, positional encoding [cite], to help MLPs overcome spectral bias [cite] }
An image can then be rendered from the predicted colour and opacities using Volumetric Rendering~\cite{nerf}.
Since neural networks enable variable spatial precision, neural radiance field methods are able to perform new-view synthesis with high-fidelity. 
% \AT{I don't think this is correct, NN give variable spatial precision vs. grids, which is why they look so sharp, and differentiability, which makes them easy to optimize.}

Naively, NeRFs only optimize a photometric loss to do multi-view 3D reconstruction, without optimizing the camera poses.
Recent methods such as BARF \cite{barf}, and NeRF\texttt{-{}-} \cite{nerfmm}, show how camera poses can be finetuned during training by directly 
using gradients from the photometric loss of the NeRF to optimize the camera poses. 
However, these camera poses must still be initialized within the vicinity of the ground-truth pose (e.g. BARF is robust to camera poses within a standard deviation of 15\textdegree).

\JZ{I think this should be called out in the intro since it's important to motivate why even noisy camera poses are valuable.}
% \TODO{what would be meaningful in reviewing NeRF, would be some formalism that shows that NeRF employs the image camera \textit{poses} in its optimization, yet \textit{does not} optimize for them natively (you can do this by having them in the math, but not in the argmin)}


